Accurate optical properties from first principles: a Quasiparticle Self consistent GW plus Bethe-Salpeter Equation approach

We present an approach to calculate the optical absorption spectra that combines the quasiparticle self-consistent GW method [Phys. Rev. B, 76 165106 (2007)] for the electronic structure with the solution of the ladder approximation to the Bethe-Salpeter equation for the macroscopic dielectric function. The solution of the Bethe-Salpeter equation has been implemented within an all-electron framework, using a linear muffin-tin orbital basis set, with the contribution from the non-local self-energy to the transition dipole moments (in the optical limit) evaluated explicitly. This approach addresses those systems whose electronic structure is poorly described within the standard perturbative GW approaches with as a starting point density-functional theory calculations. The merits of this approach have been exemplified by calculating optical absorption spectra of a strongly correlated transition metal oxide, NiO, and a narrow gap semiconductor, Ge. In both cases, the calculated spectrum is in good agreement with the experiment. It is also shown that for systems whose electronic structure is well-described within the standard perturbative GW, such as Si, LiF and h-BN, the performance of the present approach is in general comparable to the standard GW plus Bethe-Salpeter equation. It is argued that both vertex corrections to the electronic screening and the electron-phonon interaction are responsible for the observed systematic overestimation of the fundamental bandgap and spectrum onset.

==> references <==
%% This BibTeX bibliography file was created using BibDesk.
%% http://bibdesk.sourceforge.net/


%% Created for Daniel Dundas at 2010-05-27 15:58:16 +0100 

@article{QSGW_paper,
  title = {Quasiparticle self-consistent $GW$ method: A basis for the independent-particle approximation},
  author = {Kotani, Takao and van Schilfgaarde, Mark and Faleev, Sergey V.},
  journal = {Phys. Rev. B},
  volume = {76},
  issue = {16},
  pages = {165106},
  numpages = {24},
  year = {2007},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.76.165106},
  url = {http://link.aps.org/doi/10.1103/PhysRevB.76.165106}
}

@article{onida_electronic_2002,
  title = {Electronic excitations: density-functional versus many-body Green's-function approaches},
  author = {Onida, Giovanni and Reining, Lucia and Rubio, Angel},
  journal = {Rev. Mod. Phys.},
  volume = {74},
  issue = {2},
  pages = {601--659},
  numpages = {0},
  year = {2002},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/RevModPhys.74.601},
  url = {https://link.aps.org/doi/10.1103/RevModPhys.74.601}
}

@article{yambo,
title = "yambo: An ab initio tool for excited state calculations ",
journal = "Computer Physics Communications ",
volume = "180",
number = "8",
pages = "1392 - 1403",
year = "2009",
note = "",
issn = "0010-4655",
doi = "https://doi.org/10.1016/j.cpc.2009.02.003",
url = "http://www.sciencedirect.com/science/article/pii/S0010465509000472",
author = "Andrea Marini and Conor Hogan and Myrta Gr{\"u}ning and Daniele Varsano",
keywords = "Electronic structure",
keywords = "Optical properties",
keywords = "Excitons",
keywords = "Quasiparticles "
}

@article{hedin,
  title = {New Method for Calculating the One-Particle Green's Function with Application to the Electron-Gas Problem},
  author = {Hedin, Lars},
  journal = {Phys. Rev.},
  volume = {139},
  issue = {3A},
  pages = {A796--A823},
  numpages = {0},
  year = {1965},
  month = {Aug},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.139.A796},
  url = {https://link.aps.org/doi/10.1103/PhysRev.139.A796}
}
@article{QSGW_PRL,
  title = {Quasiparticle Self-Consistent $GW$ Theory},
  author = {van Schilfgaarde, M. and Kotani, Takao and Faleev, S.},
  journal = {Phys. Rev. Lett.},
  volume = {96},
  issue = {22},
  pages = {226402},
  numpages = {4},
  year = {2006},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.96.226402},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.96.226402}
}
@article{louie,
  title = {Electron correlation in semiconductors and insulators: Band gaps and quasiparticle energies},
  author = {Hybertsen, Mark S. and Louie, Steven G.},
  journal = {Phys. Rev. B},
  volume = {34},
  issue = {8},
  pages = {5390--5413},
  numpages = {0},
  year = {1986},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.34.5390},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.34.5390}
}
@article{kohnsham,
  title = {Self-Consistent Equations Including Exchange and Correlation Effects},
  author = {Kohn, W. and Sham, L. J.},
  journal = {Phys. Rev.},
  volume = {140},
  issue = {4A},
  pages = {A1133--A1138},
  numpages = {0},
  year = {1965},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.140.A1133},
  url = {https://link.aps.org/doi/10.1103/PhysRev.140.A1133}
}
@article{GW_aryasetiawan,
  author={F Aryasetiawan and O Gunnarsson},
  title={The GW method},
  journal={Reports on Progress in Physics},
  volume={61},
  number={3},
  pages={237},
  url={http://stacks.iop.org/0034-4885/61/i=3/a=002},
  year={1998},
  abstract={Calculations of ground-state and excited-state properties of materials have been one of the major goals of condensed matter physics. Ground-state properties of solids have been extensively investigated for several decades within the standard density functional theory. Excited-state properties, on the other hand, were relatively unexplored in ab initio calculations until a decade ago. The most suitable approach up to now for studying excited-state properties of extended systems is the Green function method. To calculate the Green function one requires the self-energy operator which is non-local and energy dependent. In this article we describe the GW approximation which has turned out to be a fruitful approximation to the self-energy. The Green function theory, numerical methods for carrying out the self-energy calculations, simplified schemes, and applications to various systems are described. Self-consistency issue and new developments beyond the GW approximation are also discussed as well as the success and shortcomings of the GW approximation.}
}
@article{PP_GW,
  author={Xin-Zheng Li and Ricardo Gómez-Abal and Hong Jiang and Claudia Ambrosch-Draxl and Matthias Scheffler},
  title={Impact of widely used approximations to the G 0 W 0 method: an all-electron perspective},
  journal={New Journal of Physics},
  volume={14},
  number={2},
  pages={023006},
  url={http://stacks.iop.org/1367-2630/14/i=2/a=023006},
  year={2012},
  abstract={Focusing on the fundamental band gaps in Si, diamond, BN, LiF, AlP, NaCl, CaSe and GaAs, and the semicore d-state binding energies in ZnS, ZnSe, ZnTe, CdS, CdSe, CdTe and GaN, we study the differences between the all-electron (AE) and the pseudopotential (PP)-based G 0 W 0 method. Leaving aside issues related to the choice of PPs within PP- G 0 W 0 , we analyze in detail the well-known discrepancies between AE- G 0 W 0 and PP- G 0 W 0 band gaps by separately addressing the approximations underlying PP- G 0 W 0 , i.e. the frozen-core approximation, the core-valence partitioning and the use of pseudo-wavefunctions. The largest differences, of the order of eV, appear in the exchange part of the self-energy and the exchange-correlation potential due to the core-valence partitioning. These differences cancel each other and, in doing so, make the final core-valence partitioning effect on the band gaps controllable when the semicore states are treated as valence states. This cancelation, however, is incomplete for semicore d-state binding energies, due to the strong interaction between these semicore states and the deep core. From our comprehensive analysis, we conclude that reliably describing the many-body interactions at the G 0 W 0 level and providing benchmark results require an AE treatment.}
}
@article{PP_GW2,
  title = {Influence of the Core-Valence Interaction and of the Pseudopotential Approximation on the Electron Self-Energy in Semiconductors},
  author = {G\'omez-Abal, Ricardo and Li, Xinzheng and Scheffler, Matthias and Ambrosch-Draxl, Claudia},
  journal = {Phys. Rev. Lett.},
  volume = {101},
  issue = {10},
  pages = {106404},
  numpages = {4},
  year = {2008},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.101.106404},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.101.106404}
}

@article{graphene1,
author = {Butler, Sheneve Z. and Hollen, Shawna M. and Cao, Linyou and Cui, Yi and Gupta, Jay A. and Gutiérrez, Humberto R. and Heinz, Tony F. and Hong, Seung Sae and Huang, Jiaxing and Ismach, Ariel F. and Johnston-Halperin, Ezekiel and Kuno, Masaru and Plashnitsa, Vladimir V. and Robinson, Richard D. and Ruoff, Rodney S. and Salahuddin, Sayeef and Shan, Jie and Shi, Li and Spencer, Michael G. and Terrones, Mauricio and Windl, Wolfgang and Goldberger, Joshua E.},
title = {Progress, Challenges, and Opportunities in Two-Dimensional Materials Beyond Graphene},
journal = {ACS Nano},
volume = {7},
number = {4},
pages = {2898-2926},
year = {2013},
doi = {10.1021/nn400280c},
    note ={PMID: 23464873},

URL = { 
        http://dx.doi.org/10.1021/nn400280c
    
},
eprint = { 
        http://dx.doi.org/10.1021/nn400280c
    
}

}

@Article{graphene2,
author={Wang, Qing Hua
and Kalantar-Zadeh, Kourosh
and Kis, Andras
and Coleman, Jonathan N.
and Strano, Michael S.},
title={Electronics and optoelectronics of two-dimensional transition metal dichalcogenides},
journal={Nat Nano},
year={2012},
month={Nov},
publisher={Nature Publishing Group, a division of Macmillan Publishers Limited. All Rights Reserved.},
volume={7},
number={11},
pages={699-712},
issn={1748-3387},
doi={10.1038/nnano.2012.193},
url={http://dx.doi.org/10.1038/nnano.2012.193}
}
@Article{graphene3,
author={Fiori, Gianluca
and Bonaccorso, Francesco
and Iannaccone, Giuseppe
and Palacios, Tomas
and Neumaier, Daniel
and Seabaugh, Alan
and Banerjee, Sanjay K.
and Colombo, Luigi},
title={Electronics based on two-dimensional materials},
journal={Nat Nano},
year={2014},
month={Oct},
publisher={Nature Publishing Group, a division of Macmillan Publishers Limited. All Rights Reserved.},
volume={9},
number={10},
pages={768-779},
abstract={The compelling demand for higher performance and lower power consumption in electronic systems is the main driving force of the electronics industry's quest for devices and/or architectures     based on new materials. Here, we provide a review of electronic devices based on two-dimensional materials, outlining their potential as a technological option beyond scaled complementary metal-oxide-semiconductor switches. We focus on the performance limits and advantages of these materials and associated technologies, when exploited for both digital and analog applications, focusing on the main figures of merit needed to meet industry requirements. We also discuss the use of two-dimensional materials as an enabling factor for flexible electronics and provide our perspectives on future       developments.},
note={Review},
issn={1748-3387},
url={http://dx.doi.org/10.1038/nnano.2014.207}
}

@article{GW_Ge,
  title = {Adequacy of approximations in $\mathbit{GW}$ theory},
  author = {van Schilfgaarde, Mark and Kotani, Takao and Faleev, Sergey V.},
  journal = {Phys. Rev. B},
  volume = {74},
  issue = {24},
  pages = {245125},
  numpages = {16},
  year = {2006},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.74.245125},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.74.245125}
}

@article{albrecht_GW,
  title = {Ab Initio},
  author = {Albrecht, Stefan and Reining, Lucia and Del Sole, Rodolfo and Onida, Giovanni},
  journal = {Phys. Rev. Lett.},
  volume = {80},
  issue = {20},
  pages = {4510--4513},
  numpages = {0},
  year = {1998},
  month = {May},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.80.4510},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.80.4510}
}

@article{QSGW_prl1,
  title = {All-Electron Self-Consistent $GW$ Approximation: Application to Si, MnO, and NiO},
  author = {Faleev, Sergey V. and van Schilfgaarde, Mark and Kotani, Takao},
  journal = {Phys. Rev. Lett.},
  volume = {93},
  issue = {12},
  pages = {126406},
  numpages = {4},
  year = {2004},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.93.126406},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.93.126406}
}

@article{opt_mat_el,
  title = {Optical properties of semiconductors within the independent-quasiparticle approximation},
  author = {Del Sole, R. and Girlanda, Raffaello},
  journal = {Phys. Rev. B},
  volume = {48},
  issue = {16},
  pages = {11789--11795},
  numpages = {0},
  year = {1993},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.48.11789},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.48.11789}
}

@article{opt_mat_el2,
  title = {Linear optical response in silicon and germanium including self-energy effects},
  author = {Levine, Zachary H. and Allan, Douglas C.},
  journal = {Phys. Rev. Lett.},
  volume = {63},
  issue = {16},
  pages = {1719--1722},
  numpages = {0},
  year = {1989},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.63.1719},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.63.1719}
}
@article{Hanke_mod,
author = { W.   Hanke },
title = {Dielectric theory of elementary excitations in crystals},
journal = {Advances in Physics},
volume = {27},
number = {2},
pages = {287-341},
year = {1978},
doi = {10.1080/00018737800101384},

URL = { 
        http://dx.doi.org/10.1080/00018737800101384
    
},
eprint = { 
        http://dx.doi.org/10.1080/00018737800101384
    
}

}

@article{fusion,
title = "Fusion of the LAPW and LMTO methods: The augmented plane wave plus muffin-tin orbital method",
author = "Takao Kotani and {Van Schilfgaarde}, Mark",
year = "2010",
month = "3",
doi = "10.1103/PhysRevB.81.125117",
volume = "81",
pages = "--",
journal = "Physical Review B (Condensed Matter and Materials Physics)",
issn = "1098-0121",
publisher = "American Institute of Physics",
number = "12",
}
@Inbook{methfessel_lmto,
author="Methfessel, M.
and van Schilfgaarde, M.
and Casali, R. A.",
editor="Dreyss{\'e}, Hugues",
title="A Full-Potential LMTO Method Based on Smooth Hankel Functions",
bookTitle="Electronic Structure and Physical Properies of Solids: The Uses of the LMTO Method Lectures of a Workshop Held at Mont Saint Odile, France, October 2--5,1998",
year="2000",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="114--147",
isbn="978-3-540-46437-2",
doi="10.1007/3-540-46437-9_3",
url="http://dx.doi.org/10.1007/3-540-46437-9_3"
}
@article{OKA,
  title = {Linear methods in band theory},
  author = {Andersen, O. Krogh},
  journal = {Phys. Rev. B},
  volume = {12},
  issue = {8},
  pages = {3060--3083},
  numpages = {0},
  year = {1975},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.12.3060},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.12.3060}
}
@article{kotani_MPB,
author = { Takao Kotani},
title = {Quasiparticle Self-Consistent GW Method Based on the Augmented Plane-Wave and Muffin-Tin Orbital Method},
journal = {Journal of the Physical Society of Japan},
volume = {83},
number = {9},
pages = {094711},
year = {2014},
doi = {10.7566/JPSJ.83.094711},

URL = { 
        http://dx.doi.org/10.7566/JPSJ.83.094711
    
},
eprint = { 
        http://dx.doi.org/10.7566/JPSJ.83.094711
    
}

}

@article{friedrich_paper,
  title = {Efficient implementation of the $GW$ approximation within the all-electron FLAPW method},
  author = {Friedrich, Christoph and Bl\"ugel, Stefan and Schindlmayr, Arno},
  journal = {Phys. Rev. B},
  volume = {81},
  issue = {12},
  pages = {125102},
  numpages = {16},
  year = {2010},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.81.125102},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.81.125102}
}

@article{TD_myrta,
author = {Gr{\"u}ning, Myrta and Marini, Andrea and Gonze, Xavier},
title = {Exciton-Plasmon States in Nanoscale Materials: Breakdown of the TammDancoff Approximation},
journal = {Nano Letters},
volume = {9},
number = {8},
pages = {2820-2824},
year = {2009},
doi = {10.1021/nl803717g},
    note ={PMID: 19637906},

URL = { 
        http://dx.doi.org/10.1021/nl803717g
    
},
eprint = { 
        http://dx.doi.org/10.1021/nl803717g
    
}

}

@article{BSE_paper,
  title = {A Relativistic Equation for Bound-State Problems},
  author = {Salpeter, E. E. and Bethe, H. A.},
  journal = {Phys. Rev.},
  volume = {84},
  issue = {6},
  pages = {1232--1242},
  numpages = {0},
  year = {1951},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.84.1232},
  url = {https://link.aps.org/doi/10.1103/PhysRev.84.1232}
}
@article{SC_BE,
  title = {Comment on ``Band-Gap Problem in Semiconductors Revisited: Effects of Core States and Many-Body Self-Consistency''},
  author = {Delaney, Kris and Garc\'{\i}a-Gonz\'alez, P. and Rubio, Angel and Rinke, Patrick and Godby, R. W.},
  journal = {Phys. Rev. Lett.},
  volume = {93},
  issue = {24},
  pages = {249701},
  numpages = {1},
  year = {2004},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.93.249701},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.93.249701}
}

@article{SC_EG,
  title = {Fully self-consistent $\mathrm{GW}$ self-energy of the electron gas},
  author = {Holm, B. and von Barth, U.},
  journal = {Phys. Rev. B},
  volume = {57},
  issue = {4},
  pages = {2108--2117},
  numpages = {0},
  year = {1998},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.57.2108},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.57.2108}
}
@article{SC_ener,
  title = {Quasiparticle energies for cubic BN, BP, and BAs},
  author = {Surh, Michael P. and Louie, Steven G. and Cohen, Marvin L.},
  journal = {Phys. Rev. B},
  volume = {43},
  issue = {11},
  pages = {9126--9132},
  numpages = {0},
  year = {1991},
  month = {Apr},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.43.9126},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.43.9126}
}
@article{Schwinger,
author = {Schwinger, Julian}, 
title = {On the Greens functions of quantized fields. I},
volume = {37}, 
number = {7}, 
pages = {452-455}, 
year = {1951}, 
doi = {10.1073/pnas.37.7.452}, 
URL = {http://www.pnas.org/content/37/7/452.short}, 
eprint = {http://www.pnas.org/content/37/7/452.full.pdf}, 
journal = {Proceedings of the National Academy of Sciences} 
}

@article{schwinger2,
  title = {Theory of Many-Particle Systems. I},
  author = {Martin, Paul C. and Schwinger, Julian},
  journal = {Phys. Rev.},
  volume = {115},
  issue = {6},
  pages = {1342--1373},
  numpages = {0},
  year = {1959},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRev.115.1342},
  url = {https://link.aps.org/doi/10.1103/PhysRev.115.1342}
}
@article{lif136,
title = "Electronic spectrum of crystalline lithium fluoride",
journal = "Journal of Physics and Chemistry of Solids",
volume = "28",
number = "8",
pages = "1507 - 1515",
year = "1967",
note = "",
issn = "0022-3697",
doi = "http://dx.doi.org/10.1016/0022-3697(67)90280-6",
url = "http://www.sciencedirect.com/science/article/pii/0022369767902806",
author = "D.M. Roessler and W.C. Walker",

}

@article{lif_gap,
  title = {Many-body effects on bandwidths in ionic, noble gas, and molecular solids},
  author = {Shirley, Eric L.},
  journal = {Phys. Rev. B},
  volume = {58},
  issue = {15},
  pages = {9579--9583},
  numpages = {0},
  year = {1998},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.58.9579},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.58.9579}
}

@article{lif_exp,
  title = {Electron-Hole Excitations in Semiconductors and Insulators},
  author = {Rohlfing, Michael and Louie, Steven G.},
  journal = {Phys. Rev. Lett.},
  volume = {81},
  issue = {11},
  pages = {2312--2315},
  numpages = {0},
  year = {1998},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.81.2312},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.81.2312}
}

@article{Si_exp2,
  title = {Dielectric functions and optical parameters of Si, Ge, GaP, GaAs, GaSb, InP, InAs, and InSb from 1.5 to 6.0 eV},
  author = {Aspnes, D. E. and Studna, A. A.},
  journal = {Phys. Rev. B},
  volume = {27},
  issue = {2},
  pages = {985--1009},
  numpages = {0},
  year = {1983},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.27.985},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.27.985}
}

@article{lif_seps,
  title = {Bond-orbital theory of linear and nonlinear electronic response in ionic crystals. I. Linear response},
  author = {Lines, M. E.},
  journal = {Phys. Rev. B},
  volume = {41},
  issue = {6},
  pages = {3372--3382},
  numpages = {0},
  year = {1990},
  month = {Feb},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.41.3372},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.41.3372}
}

@article{PhysRevB.64.035104,
  title = {Optical properties of BN in cubic and layered hexagonal phases},
  author = {Cappellini, Giancarlo and Satta, Guido and Palummo, Maurizia and Onida, Giovanni},
  journal = {Phys. Rev. B},
  volume = {64},
  issue = {3},
  pages = {035104},
  numpages = {11},
  year = {2001},
  month = {Jun},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.64.035104},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.64.035104}
}

@article{hbn_marini,
author = {Ludger Wirtz and Andrea Marini and Angel Rubio},
title = {Optical Absorption of hexagonal Boron Nitride and BN nanotubes},
journal = {AIP Conference Proceedings},
volume = {786},
number = {1},
pages = {391-395},
year = {2005},
}

@article{PhysRevB.87.035404,
  title = {Electronic structure of boron nitride sheets doped with carbon from first-principles calculations},
  author = {Berseneva, Natalia and Gulans, Andris and Krasheninnikov, Arkady V. and Nieminen, Risto M.},
  journal = {Phys. Rev. B},
  volume = {87},
  issue = {3},
  pages = {035404},
  numpages = {9},
  year = {2013},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.87.035404},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.87.035404}
}

@article{PhysRevLett.96.026402,
  title = {Huge Excitonic Effects in Layered Hexagonal Boron Nitride},
  author = {Arnaud, B. and Leb\`egue, S. and Rabiller, P. and Alouani, M.},
  journal = {Phys. Rev. Lett.},
  volume = {96},
  issue = {2},
  pages = {026402},
  numpages = {4},
  year = {2006},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.96.026402},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.96.026402}
}


@article{PhysRevLett.100.189701,
  title = {Comment on ``Huge Excitonic Effects in Layered Hexagonal Boron Nitride''},
  author = {Wirtz, Ludger and Marini, Andrea and Gr\"uning, Myrta and Attaccalite, Claudio and Kresse, Georg and Rubio, Angel},
  journal = {Phys. Rev. Lett.},
  volume = {100},
  issue = {18},
  pages = {189701},
  numpages = {1},
  year = {2008},
  month = {May},
  publisher = {American Physical Society},
}


@ARTICLE{2005cond.mat..8421W,
   author = {{Wirtz}, L. and {Marini}, A. and {Gr{\"u}ning}, M. and {Rubio}, A.
	},
    title = "{Excitonic effects in optical absorption and electron-energy loss spectra of hexagonal boron nitride}",
  journal = {eprint arXiv:cond-mat/0508421},
   eprint = {cond-mat/0508421},
 keywords = {Condensed Matter - Materials Science},
     year = 2005,
    month = aug,
   adsurl = {http://adsabs.harvard.edu/abs/2005cond.mat..8421W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Watanabe2004,
annote = {10.1038/nmat1134},
author = {Watanabe, Kenji and Taniguchi, Takashi and Kanda, Hisao},
issn = {1476-1122},
journal = {Nat Mater},
month = {jun},
number = {6},
pages = {404--409},
title = {{Direct-bandgap properties and evidence for ultraviolet lasing of hexagonal boron nitride single crystal}},
url = {http://dx.doi.org/10.1038/nmat1134},
volume = {3},
year = {2004}
}


@article{hbn_exp,
  title = {Interband transitions, plasmons, and dispersion in hexagonal boron nitride},
  author = {Tarrio, C. and Schnatterly, S. E.},
  journal = {Phys. Rev. B},
  volume = {40},
  issue = {11},
  pages = {7852--7859},
  numpages = {0},
  year = {1989},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.40.7852},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.40.7852}
}

@Book{ kittel,
title = { Introduction to solid state physics },
author = { Charles Kittel },
url = { http://openlibrary.org/books/OL3302328M },
publisher = { Hoboken, NJ Wiley },
year = { 2005 },
type = { Book },
edition = { 8th ed },
isbn = { 047141526X },
subjects = { Solid state physics },
note = { Includes bibliographical references and index.
"Chapter 18, Nanostructures, was written by Professor Paul McEuen ..." },
catalogue-url = { http://trove.nla.gov.au/work/9250395 }
}

@article{vasp,
  title = {Ab initio},
  author = {Kresse, G. and Hafner, J.},
  journal = {Phys. Rev. B},
  volume = {47},
  issue = {1},
  pages = {558--561},
  numpages = {0},
  year = {1993},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.47.558},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.47.558}
}
@article{espresso,
  author={Paolo Giannozzi and Stefano Baroni and Nicola Bonini and Matteo Calandra and Roberto Car and Carlo Cavazzoni and Davide
Ceresoli and Guido L Chiarotti and Matteo Cococcioni and Ismaila Dabo and Andrea Dal Corso and Stefano de
Gironcoli and Stefano Fabris and Guido Fratesi and Ralph Gebauer and Uwe Gerstmann and Christos Gougoussis and Anton
Kokalj and Michele Lazzeri and Layla Martin-Samos and Nicola Marzari and Francesco Mauri and Riccardo Mazzarello and Stefano
Paolini and Alfredo Pasquarello and Lorenzo Paulatto and Carlo Sbraccia and Sandro Scandolo and Gabriele Sclauzero and Ari P
Seitsonen and Alexander Smogunov and Paolo Umari and Renata M Wentzcovitch},
  title={QUANTUM ESPRESSO: a modular and open-source software project for quantum simulations of materials},
  journal={Journal of Physics: Condensed Matter},
  volume={21},
  number={39},
  pages={395502},
  url={http://stacks.iop.org/0953-8984/21/i=39/a=395502},
  year={2009},
  abstract={QUANTUM ESPRESSO is an integrated suite of computer codes for electronic-structure calculations and materials modeling, based on density-functional theory, plane waves, and pseudopotentials (norm-conserving, ultrasoft, and projector-augmented wave). The acronym ESPRESSO stands for opEn Source Package for Research in Electronic Structure, Simulation, and Optimization . It is freely available to researchers around the world under the terms of the GNU General Public License. QUANTUM ESPRESSO builds upon newly-restructured electronic-structure codes that have been developed and tested by some of the original authors of novel electronic-structure algorithms and applied in the last twenty years by some of the leading materials modeling groups worldwide. Innovation and efficiency are still its main focus, with special attention paid to massively parallel architectures, and a great effort being devoted to user friendliness. QUANTUM ESPRESSO is evolving towards a distribution of independent and interoperable codes in the spirit of an open-source project, where researchers active in the field of electronic-structure calculations are encouraged to participate in the project by contributing their own codes or by implementing their own ideas into existing codes.}
}
@article{Phonons,
  title = {Effects of Electronic and Lattice Polarization on the Band Structure of Delafossite Transparent Conductive Oxides},
  author = {Vidal, Julien and Trani, Fabio and Bruneval, Fabien and Marques, Miguel A. L. and Botti, Silvana},
  journal = {Phys. Rev. Lett.},
  volume = {104},
  issue = {13},
  pages = {136401},
  numpages = {4},
  year = {2010},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.104.136401},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.104.136401}
}
@misc{questaal_web,
  title = {Questaal code website},
  howpublished = {\url{https://www.questaal.org}},
  note = {Accessed: 2017-07-04. Our $GW$ implementation was adapted from the original ecalj package, now at \url{https://github.com/tkotani/ecalj/}.
}
}
@article{ge_paper,
  title = {Band-Gap Problem in Semiconductors Revisited: Effects of Core States and Many-Body Self-Consistency},
  author = {Ku, Wei and Eguiluz, Adolfo G.},
  journal = {Phys. Rev. Lett.},
  volume = {89},
  issue = {12},
  pages = {126401},
  numpages = {4},
  year = {2002},
  month = {Aug},
  publisher = {American Physical Society},
}
@article{PhysRevLett.55.418,
  title = {Band gaps and electronic structure of transition-metal compounds},
  author = {Zaanen, J. and Sawatzky, G. A. and Allen, J. W.},
  journal = {Phys. Rev. Lett.},
  volume = {55},
  issue = {4},
  pages = {418--421},
  numpages = {0},
  year = {1985},
  month = {Jul},
  publisher = {American Physical Society},
}
@article{ge_comm,
  title = {Comment on ``Band-Gap Problem in Semiconductors Revisited: Effects of Core States and Many-Body Self-Consistency''},
  author = {Delaney, Kris and García-Gonz{'a}lez, P. and  Rubio, Angel and Rinke, Patrick and Godby, R. W.},
  journal = {Phys. Rev. Lett.},
  volume = {93},
  issue = {24},
  pages = {249701},
  numpages = {},
  year = {2004},
  month = {Dec},
  publisher = {American Physical Society},
}
@article{ge_exp,
  title = {Dielectric functions and optical parameters of Si, Ge, GaP, GaAs, GaSb, InP, InAs, and InSb from 1.5 to 6.0 eV},
  author = {Aspnes, D. E. and Studna, A. A.},
  journal = {Phys. Rev. B},
  volume = {27},
  issue = {2},
  pages = {985--1009},
  numpages = {0},
  year = {1983},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.27.985},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.27.985}
}
@article{Ge_gap2,
  title = {Core polarization in semiconductors: Effects on quasiparticle energies},
  author = {Shirley, Eric L. and Zhu, Xuejun and Louie, Steven G.},
  journal = {Phys. Rev. Lett.},
  volume = {69},
  issue = {20},
  pages = {2955--2958},
  numpages = {0},
  year = {1992},
  month = {Nov},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.69.2955},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.69.2955}
}
@article{semicore1,
  title = {Role of semicore $d$ electrons in quasiparticle band-structure calculations},
  author = {Rohlfing, Michael and Kr\"uger, Peter and Pollmann, Johannes},
  journal = {Phys. Rev. B},
  volume = {57},
  issue = {11},
  pages = {6485--6492},
  numpages = {0},
  year = {1998},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.57.6485},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.57.6485}
}
@article{MARQUES20122272,
title = "Libxc: A library of exchange and correlation functionals for density functional theory",
journal = "Computer Physics Communications",
volume = "183",
number = "10",
pages = "2272 - 2281",
year = "2012",
note = "",
issn = "0010-4655",
author = "Miguel A.L. Marques and Micael J.T. Oliveira and Tobias Burnus",
keywords = "Density functional theory",
keywords = "Density functionals",
keywords = "Local density approximation",
keywords = "Generalized gradient approximation",
keywords = "Hybrid functionals"
}

@article{PhysRevB.37.10159,
  title = {Self-energy operators and exchange-correlation potentials in semiconductors},
  author = {Godby, R. W. and Schl\"uter, M. and Sham, L. J.},
  journal = {Phys. Rev. B},
  volume = {37},
  issue = {17},
  pages = {10159--10175},
  numpages = {0},
  year = {1988},
  month = {Jun},
  publisher = {American Physical Society},
}

@article{AULBUR20001,
title = "Quasiparticle Calculations in Solids",
journal = "Solid State Physics",
volume = "54",
number = "",
pages = "1 - 218",
year = "2000",
note = "",
issn = "0081-1947",
author = "Wilfried G. Aulbur and Lars Jnsson and John W. Wilkins"
}

@article{PhysRev.139.A796,
  title = {New Method for Calculating the One-Particle Green's Function with Application to the Electron-Gas Problem},
  author = {Hedin, Lars},
  journal = {Phys. Rev.},
  volume = {139},
  issue = {3A},
  pages = {A796--A823},
  numpages = {0},
  year = {1965},
  month = {Aug},
  publisher = {American Physical Society}
  }

@article {PSSB:PSSB200945204,
author = {Schleife, A. and Fuchs, F. and Rdl, C. and Furthmller, J. and Bechstedt, F.},
title = {Band-structure and optical-transition parameters of wurtzite MgO, ZnO, and CdO from quasiparticle calculations},
journal = {physica status solidi (b)},
volume = {246},
number = {9},
publisher = {WILEY-VCH Verlag},
issn = {1521-3951},
pages = {2150--2153},
keywords = {71.15.-m, 71.20.Nr, 71.35.Cc, 71.70.Ej},
year = {2009}
}

@article{PhysRevLett.99.266402,
  title = {Understanding Correlations in Vanadium Dioxide from First Principles},
  author = {Gatti, Matteo and Bruneval, Fabien and Olevano, Valerio and Reining, Lucia},
  journal = {Phys. Rev. Lett.},
  volume = {99},
  issue = {26},
  pages = {266402},
  numpages = {4},
  year = {2007},
  month = {Dec},
  publisher = {American Physical Society}
}

@article{PhysRevLett.91.176402,
  title = {Dynamical Excitonic Effects in Metals and Semiconductors},
  author = {Marini, Andrea and Del Sole, Rodolfo},
  journal = {Phys. Rev. Lett.},
  volume = {91},
  issue = {17},
  pages = {176402},
  numpages = {4},
  year = {2003},
  month = {Oct},
  publisher = {American Physical Society}
}



@article{doi:10.1063/1.2189226,
author = {Myrta Gr{\"u}ning and Andrea Marini and Angel Rubio},
title = {Density functionals from many-body perturbation theory: The band gap for semiconductors and insulators},
journal = {The Journal of Chemical Physics},
volume = {124},
number = {15},
pages = {154108},
year = {2006}
}

}

@ARTICLE{Vidal10,
   author = "Julien Vidal and Silvana Botti and Pr Olsson and Jean-Franois Guillemoles and Lucia Reining",
   year = "2010",
   journal = "Phys. Rev. Lett.",
   title = {{Strong Interplay between Structure and Electronic Properties in CuInSe$_{2}$: A First-Principles Study}},
   volume = "104",
   pages = "056401",
   anote = {},
   abstract = {}
}

@ARTICLE{mark06adeq,
   author = "M. van Schilfgaarde and T.  Kotani and S.  V.  Faleev",
   year = "2006",
   journal = "Phys. Rev. B",
   title = {{Adequacy of approximations in {\emph{GW}} theory}},
   volume = "74",
   pages = "245125"
}

@Article{Shirley96,
  title = {Self-consistent GW and higher-order calculations of electron states in metals},
  author = {Shirley, Eric L.},
  journal = {Phys. Rev. B},
  volume = {54},
  number = {11},
  pages = {7758--7764},
  numpages = {6},
  year = {1996},
  month = {Sep},
  doi = {10.1103/PhysRevB.54.7758},
  publisher = {American Physical Society},
  abstract = {Past work, treating simple metals in the GW
  approximation, has largely neglected effects of self-consistency and
  higher-order vertex corrections on occupied bandwidths. This work
  presents self-consistent GW results, plus nearly self-consistent
  higher-order results, for jellium, illustrating that both effects
  are large, yet largely canceling (e.g., 0.65-eV effects on the
  sodium bandwidth, but a combined effect of only 0.13 eV). This
  supports findings that many-body effects substantially reduce such
  bandwidths.}
}

@ARTICLE{Belashchenko06,
   author = "K. D. Belashchenko and V. P. Antropov and N. E. Zein",
   year = "2006",
   journal = "Phys. Rev. B",
   title = {{Self-consistent local {GW} method: {A}pplication to 3d and 4d metals}},
   volume = "73",
   pages = "073105"
}

@ARTICLE{2017arXiv170909194B,
   author = {{Bhandari}, C. and {van Schilfgaarde}, M. and {Kotani}, T. and 
{Lambrecht}, W.~R.~L.},
    title = "{All-electron quasi-particle self-consistent $GW$ band structures for SrTiO$\_3$ including lattice polarization corrections in different phase}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1709.09194},
 primaryClass = "cond-mat.mtrl-sci",
 keywords = {Condensed Matter - Materials Science},
     year = 2017,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170909194B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Bruneval06b,
   author = "Fabien Bruneval and Nathalie Vast and Lucia Reining and M. Izquierdo and F. Sirotti and N. Barrett",
   year = "2006",
   journal = "Phys. Rev. Lett.",
   title = {{Exchange and Correlation Effects in Electronic Excitations of Cu$_{2}$O}},
   volume = "97",
   pages = "267601",
   anote = {},
   abstract = {State-of-the-art theoretical methods fail in describing
   the optical absorption spectrum, band gap, and optical onset of
   Cu2O. We have extended a recently proposed self-consistent
   quasiparticle approach, based on the GW approximation, to the
   calculation of optical spectra, including excitonic effects. The
   band structure compares favorably with our present angle-resolved
   photoemission measurements. The excitonic effects based on these
   realistic band structure and screening provide a reliable optical
   absorption spectrum, which allows for a revised interpretation of
   its main structures.}
}

@article{Cassabois2016,
author = {Cassabois, G and Valvin, P and Gil, B},
month = {jan},
pages = {262},
publisher = {Nature Publishing Group},
title = {{Hexagonal boron nitride is an indirect bandgap semiconductor}},
volume = {10},
year = {2016}
}

@article{SOLOZHENKO20011331,
author = {Solozhenko, V L and Lazarenko, A G and Petitet, J.-P. and Kanaev, A V},
doi = {https://doi.org/10.1016/S0022-3697(01)00030-0},
issn = {0022-3697},
journal = {Journal of Physics and Chemistry of Solids},
keywords = {A. Semiconductors,D. Luminescence},
number = {7},
pages = {1331--1334},
title = {{Bandgap energy of graphite-like hexagonal boron nitride}},
volume = {62},
year = {2001}
}

@article{PhysRevLett.101.106405,
  title = {Ab Initio},
  author = {Marini, Andrea},
  journal = {Phys. Rev. Lett.},
  volume = {101},
  issue = {10},
  pages = {106405},
  numpages = {4},
  year = {2008},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.101.106405},
}


@article {hBN_BE,
author = {Museur, L. and Brasse, G. and Pierret, A. and Maine, S. and Attal-Tretout, B. and Ducastelle, F. and Loiseau, A. and Barjon, J. and Watanabe, K. and Taniguchi, T. and Kanaev, A.},
title = {Exciton optical transitions in a hexagonal boron nitride single crystal},
journal = {physica status solidi (RRL) - Rapid Research Letters},
volume = {5},
number = {5-6},
publisher = {WILEY-VCH Verlag},
issn = {1862-6270},
url = {http://dx.doi.org/10.1002/pssr.201105190},
doi = {10.1002/pssr.201105190},
pages = {214--216},
keywords = {hexagonal boron nitride, photoluminescence, photoconductivity, excitons, band gap},
year = {2011},
}

@article{deriv_disc,
  title = {Band-gap energy in the random-phase approximation to density-functional theory},
  author = {Niquet, Y. M. and Gonze, X.},
  journal = {Phys. Rev. B},
  volume = {70},
  issue = {24},
  pages = {245115},
  numpages = {12},
  year = {2004},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.70.245115},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.70.245115}
}

@article{PhysRevB.13.5530,
  title = {Thermoreflectance of LiF between 12 and 30 eV},
  author = {Piacentini, M. and Lynch, D. W. and Olson, C. G.},
  journal = {Phys. Rev. B},
  volume = {13},
  issue = {12},
  pages = {5530--5543},
  numpages = {0},
  year = {1976},
  month = {Jun},
}

@article{Roessler:67,
author = {D. M. Roessler and W. C Walker},
journal = {J. Opt. Soc. Am.},
keywords = {},
number = {6},
pages = {835--836},
publisher = {OSA},
title = {Optical Constants of Magnesium Oxide and Lithium Fluoride in the Far Ultraviolet$\ast$},
volume = {57},
month = {Jun},
year = {1967},
}

@article{Dauer:00,
author = {V\'{e}ronique Dauer},
journal = {J. Opt. Soc. Am. B},
keywords = {Optical constants; Optical properties; Ultraviolet, vacuum ; Thin films},
number = {2},
pages = {300--303},
publisher = {OSA},
title = {Optical constants of lithium fluoride thin films in the far ultraviolet},
volume = {17},
month = {Feb},
year = {2000},
}


@article{PhysRev.136.B864,
  title = {Inhomogeneous Electron Gas},
  author = {Hohenberg, P. and Kohn, W.},
  journal = {Phys. Rev.},
  volume = {136},
  issue = {3B},
  pages = {B864--B871},
  numpages = {0},
  year = {1964},
  month = {Nov},
}


@article{ISI:000258905700014,
author = {Abbamonte, Peter and Graber, Tim and Reed, James P. and Smadici, Serban and Yeh, Chen-Lin and Shukla, Abhay and Rueff, Jean-Pascal and Ku, Wei},
title = {Dynamical reconstruction of the exciton in LiF with inelastic x-ray scattering},
journal = {PNAS},
year = {2008},
volume = {105},
number = {34},
pages = {12159-12163},
}

@article{phonons_walt,
  title = {Lattice polarization effects on the screened Coulomb interaction $W$ of the $GW$ approximation},
  author = {Lambrecht, Walter R. L. and Bhandari, Churna and van Schilfgaarde, Mark},
  journal = {Phys. Rev. Materials},
  volume = {1},
  issue = {4},
  pages = {043802},
  numpages = {7},
  year = {2017},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevMaterials.1.043802},
  url = {https://link.aps.org/doi/10.1103/PhysRevMaterials.1.043802}
}
@article{hbn_bs,
  title = {Exciton energy-momentum map of hexagonal boron nitride},
  author = {Fugallo, Giorgia and Aramini, Matteo and Koskelo, Jaakko and Watanabe, Kenji and Taniguchi, Takashi and Hakala, Mikko and Huotari, Simo and Gatti, Matteo and Sottile, Francesco},
  journal = {Phys. Rev. B},
  volume = {92},
  issue = {16},
  pages = {165122},
  numpages = {5},
  year = {2015},
  month = {Oct},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.92.165122},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.92.165122}
}
@article{NiO_exp,
  title = {Magnitude and Origin of the Band Gap in NiO},
  author = {Sawatzky, G. A. and Allen, J. W.},
  journal = {Phys. Rev. Lett.},
  volume = {53},
  issue = {24},
  pages = {2339--2342},
  numpages = {0},
  year = {1984},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.53.2339},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.53.2339}
}
@article{PhysRevB.47.2130,
  title = {Inverse-photoemission study of Ge(100), Si(100), and GaAs(100): Bulk bands and surface states},
  author = {Ortega, J. E. and Himpsel, F. J.},
  journal = {Phys. Rev. B},
  volume = {47},
  issue = {4},
  pages = {2130--2137},
  numpages = {0},
  year = {1993},
  month = {Jan},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.47.2130},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.47.2130}
}

@article{PhysRevB.36.4821,
  title = {Temperature dependence of the dielectric function and interband critical points in silicon},
  author = {Lautenschlager, P. and Garriga, M. and Vina, L. and Cardona, M.},
  journal = {Phys. Rev. B},
  volume = {36},
  issue = {9},
  pages = {4821--4830},
  numpages = {0},
  year = {1987},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.36.4821},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.36.4821}
}

@article{NiO_expopt,
  title = {Optical Properties of NiO and CoO},
  author = {Powell, R. J. and Spicer, W. E.},
  journal = {Phys. Rev. B},
  volume = {2},
  issue = {6},
  pages = {2182--2193},
  numpages = {0},
  year = {1970},
  month = {Sep},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevB.2.2182},
  url = {https://link.aps.org/doi/10.1103/PhysRevB.2.2182}
}

@article{Liang2010,
author = {Liang, Di and Bowers, John E},
journal = {Nature Photonics},
month = {jul},
pages = {511},
publisher = {Nature Publishing Group, a division of Macmillan Publishers Limited. All Rights Reserved.},
title = {{Recent progress in lasers on silicon}},
url = {http://dx.doi.org/10.1038/nphoton.2010.167 http://10.0.4.14/nphoton.2010.167},
volume = {4},
year = {2010}
}

@article{PhysRevLett.99.246403,
  title = {Accurate Quasiparticle Spectra from Self-Consistent GW Calculations with Vertex Corrections},
  author = {Shishkin, M. and Marsman, M. and Kresse, G.},
  journal = {Phys. Rev. Lett.},
  volume = {99},
  issue = {24},
  pages = {246403},
  numpages = {4},
  year = {2007},
  month = {Dec},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevLett.99.246403},
  url = {https://link.aps.org/doi/10.1103/PhysRevLett.99.246403}
}

@incollection{GROSSO2000230,
title = "\{VII\} - Excitons, plasmons and dielectric screening in crystals ",
editor = "GROSSO, GIUSEPPE  and PARRAVICINI, GIUSEPPE PASTORI ",
booktitle = "Solid State Physics ",
publisher = "Academic Press",
edition = "",
address = "London",
year = "2000",
pages = "230 - 267",
isbn = "978-0-12-304460-0",
doi = "https://doi.org/10.1016/B978-012304460-0/50007-4",
url = "https://www.sciencedirect.com/science/article/pii/B9780123044600500074",
author = "GIUSEPPE GROSSO and GIUSEPPE PASTORI PARRAVICINI"
}

